SBOM.EXE: Countering Dynamic Code Injection based on Software Bill of Materials in Java

Software supply chain attacks have become a significant threat as software development increasingly relies on contributions from multiple, often unverified sources. The code from unverified sources does not pose a threat until it is executed. Log4Shell is a recent example of a supply chain attack that processed a malicious input at runtime, leading to remote code execution. It exploited the dynamic class loading facilities of Java to compromise the runtime integrity of the application. Traditional safeguards can mitigate supply chain attacks at build time, but they have limitations in mitigating runtime threats posed by dynamically loaded malicious classes. This calls for a system that can detect these malicious classes and prevent their execution at runtime. This paper introduces SBOM.EXE, a proactive system designed to safeguard Java applications against such threats. SBOM.EXE constructs a comprehensive allowlist of permissible classes based on the complete software supply chain of the application. This allowlist is enforced at runtime, blocking any unrecognized or tampered classes from executing. We assess SBOM.EXE's effectiveness by mitigating 3 critical CVEs based on the above threat. We run our tool with 3 open-source Java applications and report that our tool is compatible with real-world applications with minimal performance overhead. Our findings demonstrate that SBOM.EXE can effectively maintain runtime integrity with minimal performance impact, offering a novel approach to fortifying Java applications against dynamic classloading attacks.

==> old-text.tex <==
%4.2

The core idea in the \texttt{Indexing} phase is to list all Java classes necessary to run the application.
The Indexing phase is done before the application is deployed to production.
Indexing is performed in a secure and trusted environment so it ensures that no malicious code is added to the list, see \autoref{sec:threat-model}.

In Java, there are three types of binary classes: the environment classes, the supply chain classes, and dynamically-loaded classes~\cite{noauthor_java_nodate}.
First, environment classes are the built-in classes provided by the Java standard library.
Supply chain classes are classes written by the author and classes declared as dependencies to the application.
Finally, dynamically-loaded classes are classes that only appear at runtime from a remote source or is generated.

% indexers
The environment Indexer scans the Java standard library and records the checksum of each standard class in the \ac{BOMI}.
We rely on an \ac{SBOM} (\autoref{sec:intro-sbom}) and package managers to provide all binary classes in the supply chain.
Hence, the supply chain indexer starts by calling an \ac{SBOM} producer, in order to scan all binary classes from the supply chain, which are statically known.
The Supply Chain Indexer parses the \ac{SBOM}, downloads the binary code from the package registry, and records the checksum of each class in the \ac{BOMI}.

Finally, the dynamic code indexer runs the tests of the application in order to trigger dynamic code loading and generation, which will be explained in \autoref{sec:dynamic-code}.




If the class does not exist in \ac{BOMI}, this is considered malicious code injection.
If the class exists but the checksum does not match, the class is considered tampered.
In both cases, a termination of the application is issued through the classloader and the process running the application is shutdown. 
In addition, the incident is reported to the security team of the application.







\section{Implementation}

\subsubsection{Runtime Guard}

\todo{discuss the intention and the key concepts of runtime monitoring, checking loaded code, etc. before going into the implementation details}

The second component of \toolname is the runtime agent.
This is a Java agent that is attached to the application during startup.
Its input is both index files.
A java agent is executed \texttt{premain}, which is a special method in the agent API.
This method is executed before the main method of an application is invoked but after the JVM startup.
The main method of an application is the entry point of the application.
Therefore before the main method are no non \ac{JVM} classes loaded.
This means that the agent can safely attach to the class loading process.
During the agent initialization, we attach a \texttt{ClassFileTransformer}.
This transformer is called for every class file before it is linked.
This means that the transformer is called before the class is initialized.
In this step, the JVM only reads the class file and does not execute any code.
So we can stop the execution of the application before any untrusted code is executed.
If the JVM loads a class the agent gets metainformation about the class and the bytecode.
For this bytecode, we compute a checksum.
Then we check given the canonical name of the class if the class is in the index.
If not we terminate the application.\todo{pretty in your face, maybe more soft we do what a user wants to do?}

\subsection{\toolname usage lifecycle}
\todo{Remove? Not sure where it fits}
The \toolname usage lifecycle consists of two phases, the index phase and the runtime phase.
\begin{enumerate}
  \item \textbf{SBOM creation}: First the developer creates an SBOM for the application.
  \item \texttt{Supply Chain Index}: For the given SBOM \toolname creates a supply chain index.
  \item \texttt{Environment Index}: For the given environment \toolname creates an environment index.
  \item \textbf{Runtime phase:} In this phase, the developer attaches the agent to the application given the two index files.
\end{enumerate}
First, the developer creates an SBOM for the application.
This SBOM contains all dependencies of the application.
Afterward, the SBOM \toolname creates a supply chain index.
This index contains all dependencies and their checksums.
Then the developer creates an environment index.
This index contains all classes of the Java standard library and their checksums.
With both these index files, the developer attaches the agent to the application.
\todo{ref to figure?}


\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{fig/workflow.pdf}
  \caption{Overview of SBOM.exe design}
  \label{fig:overview}
\end{figure*}

\todo{test cases -> test suites}
\todo{load class arrow}
\todo{action is index but it produces a class allow list}
\todo{depict a malicious actor and show how it interacts with the application}
\begin{lstlisting}[backgroundcolor=\color{gray!10}, caption={An example decompiled class generated during runtime. The bytecode is decompiled using FernFlower}, label=lst:example-class,language=Java,belowskip=\baselineskip]
  public class GeneratedConstructorAccessor6 extends ConstructorAccessorImpl {
    public GeneratedConstructorAccessor6() {
    }

    public Object newInstance(Object[] var1) throws InvocationTargetException {
        jdk.proxy2.Proxy8 var10000;
        jdk.proxy2.Proxy8 var10001;
        InvocationHandler var10002;
        try {
            var10000 = new jdk.proxy2.Proxy8;
            var10001 = var10000;
            if (var1.length != 1) {
                throw new IllegalArgumentException();
            }

            var10002 = (InvocationHandler)var1[0];
        } catch (NullPointerException | ClassCastException var3) {
            throw new IllegalArgumentException(var3.toString());
        }

        try {
            var10001.<init>(var10002);
            return var10000;
        } catch (Throwable var2) {
            throw new InvocationTargetException(var2);
        }
    }
  }
\end{lstlisting}


\subsubsection{Overview}
\toolname works in two steps. First, it generates a fingerprint of the all the classfiles that are packaged into the final executable jar. Second, it attaches to the executable jar while execution and monitors for class that are being loaded. If any class loaded is not in the fingerprint, the tool terminates the execution.

\subsubsection{Input}

The tool takes in a source project which is built using maven. Optionally, it also takes in a a configuration file that contains a list of external jars.

\subsection{Classfile Fingerprinting}

The tool resolves all direct and indirect dependencies of the source project using maven.
Each maven dependency is stored as a jar file in the filesystem.
The classfiles are extracted from each jar file and its checksum is computed.
Since the project itself also contains some classfiles, we directly get it from the build directory.
There is also an option to include external jars in the fingerprint.

The fingerprint file is a line delimited JSON file with the following format:
\begin{lstlisting}
  {
   "org/example/LocalFile":[
      {
         "classFileAttributes":{
            "classfileVersion":"59.0",
            "hash":"4535b6c4b68034eb84b4a8777f20a37aaa2e47c12a024934b74e8b26bff08f45",
            "algorithm":"SHA256"
         },
         "groupId":"org.example",
         "artifactId":"url-classloader",
         "version":"1.0-SNAPSHOT"
      }
   ]
}
\end{lstlisting}

\begin{lstlisting}
  {
  "NonMalicious": [
    {
      "classFileAttributes": {
        "classfileVersion": "61.0",
        "hash": "de3318e0ba5527a90fb600307ca12e0d06752474d1da3086cfdb4a48f714da5d",
        "algorithm": "SHA256"
      },
      "path": "/home/aman/personal/who-are-you/classfile-fingerprint/target/maven-it/io/github/algomaster99/it/GenerateMojoIT/url_classloader_local_jar/project/external_source/non-malicious.jar"
    }
  ]
}
\end{lstlisting}
\subsection{Agent inside the JVM}

\todo{differentiate between the two sections by colour coding}


% figma https://www.figma.com/file/hJy2ipZIE6zxGpZl4edy20/Untitled?type=design&node-id=0%3A1&mode=design&t=hIPopkVquOTQXC0o-1

\subsection{Watchdog agent}

The watchdog agent is attached to the executable jar file using the java agent API.
The agent is loaded before the main class of the executable jar.
The agent starts a new thread which monitors for class loading events.
If a class is loaded which is not in the fingerprint, or is modified based on the hash,
the agent terminates the execution.







\section{Threat Model and Assumptions}
\label{sec:threat-model}
\TODO{@Benoit we are not sure if we should mention our approach in this section already. If we should at which subsection shall we put it?}
Our threat model is based on the guidelines provided by the OWASP \cite{noauthor_threat_nodate}.
OWASP is the Open Web Application Security Project, a nonprofit foundation that works to improve the security of software.
Their guidelines are defacto standard for software security practices.

\subsection{Description of the system to be modeled}
Our system is a Java application running in an untrusted environment.
An untrusted environment is an environment with shared resources.
This includes shared file systems, shared memory, and shared CPU.
On our system exists a Java Virtual Machine (JVM) which executes the application.
The application is packaged as an executable jar file.

\subsection{Assumptions that can be checked or challenged in the future as the threat landscape changes}
Our first assumption is a complete and correct Software Bill of Materials (SBOM).
This means that the SBOM contains all dependencies and their checksums and has been produced in a trusted environment.
Second we assume the solution itself is not compromised or tampered with.


\subsection{Potential threats to the system}
Due to the characteristics of shared resources, the JVM is vulnerable to multiple threats.
It can be attacked by executing malicious code.
The malicious code can be executed by loading a malicious class or by modifying an existing class.
These malicious classes could steal credentials or computing resources for crypto-mining.

\subsection{Actions that can be taken to mitigate each threat}
A possible action to mitigate the threat is to ensure that the application only loads classes that are known to be safe.
There exist multiple approaches for integrity checking like code signing, checksums or closed-world applications.

Code signing is a technique where the author of the code signs the code.
Before executing the code, the signature is verified and rejected if the signature is not valid.

Checksum are another technique where the checksum of the code is computed and compared against a known good value.
If the checksum does not match, the code is rejected.

A closed-world application is an application that is air-gapped and completely self-contained.
This means that the program only loads classes that are known to be safe.

\subsection{A way of validating the model and threats, and verification of success of actions taken}
A solution needs to fulfill the two criteria.
First, the application must work correctly even after a solution is applied.
Second, the solution must detect the modification of the application.
The solution is verified by running it on a set of applications with known vulnerabilities.
These vulnerabilities must be detected by the solution and mitigated.

% Not attacked:
% % - JVM \\
% % - Correct complete non attacked SBOM. \\
% % - Agent + its dependencies \\
% % - Environment \\
% Attackable:\\
% - Dependencies, classes, checksums etc.\\
% - Maven-Central can deliever malicious jars because the hash in the SBOM is not checked.\\
% 
% Guarded:\\
% We only allow loading classes that are in the SBOM or a JDK class (or level 4). \\
% Whitelist with package name is easy to attack because you can just create a class with the same package name. \\
% 
% who is malicious? when and where?
% 
% do we trust the local jar? the maven central jar? the sbom producer?
% 


